A Deep Learning Based Behavioral Approach to Indoor Autonomous Navigation

We present a semantically rich graph representation for indoor robotic navigation. Our graph representation encodes: semantic locations such as offices or corridors as nodes, and navigational behaviors such as enter office or cross a corridor as edges. In particular, our navigational behaviors operate directly from visual inputs to produce motor controls and are implemented with deep learning architectures. This enables the robot to avoid explicit computation of its precise location or the geometry of the environment, and enables navigation at a higher level of semantic abstraction. We evaluate the effectiveness of our representation by simulating navigation tasks in a large number of virtual environments. Our results show that using a simple sets of perceptual and navigational behaviors, the proposed approach can successfully guide the way of the robot as it completes navigational missions such as going to a specific office. Furthermore, our implementation shows to be effective to control the selection and switching of behaviors.

==> resultados.tex <==
\section{\label{Sec:Experiment}Experiments}
As we discuss, we test the proposed approach using simulated environments that 
resemble the configuration of office building spaces. As illustrated in Figure 
\ref{Fig:Maps}, our current implementation considers 3 types of 
office building spaces: offices, corridors, and halls. In terms of 
behaviors, while it is possible to explore automatic 
techniques to identify them \cite{Justin:EtAl:2017}\cite{NeuralTuring:2015}, 
for simplicity, we manually preselect a set of behaviors that can meet the 
navigational requirements of the intended environment. Specifically, we 
implement the following behaviors:

\begin{itemize}
 \item Follow-Corridor (\textbf{FC}): a reactive behavior able to lead 
the way of the robot as it navigates through a corridor. The input to this 
behavior is the current view of the robot (RGB image).

 \item Out-Office (\textbf{OO}): a reactive behavior able to lead the 
way of the robot as it leaves an office. The input to this behavior is the 
current view of the robot and a 3D vector encoding the direction that 
the robot should take after leaving the office: \textit{right}, 
\textit{left}, or \textit{center} \footnote{\textit{Center} indicates direct 
crossing to the office across the 
corridor.}.  

\item In-Office (\textbf{IO}): a reactive behavior able to lead the 
way of the robot as it navigates through a corridor and enters to the next 
office on its way. The input to this behavior is the 
current view of the robot and a 3D vector encoding the direction 
that the robot should take to enter the next office:  \textit{right} or 
\textit{left}.

\item Cross-Hall (\textbf{CH}): a reactive behavior able to lead the 
way of the robot as it crosses a hall. The input to this behavior is the 
current view of the robot and a 3D vector encoding the direction 
that the robot should follow to leave the corridor: \textit{right}, 
\textit{left}, or \textit{center}

\item Change-Corridor (\textbf{CC}): a reactive behavior able to lead the 
way of the robot as it faces an intersection to follow a new 
corridor. The input to this behavior is the 
current view of the robot and a 3D vector encoding the direction of the next 
corridor: \textit{right}, \textit{left}, 
or \textit{center}. 

\item Place-Detection (\textbf{PLD}): a perceptual behavior that identifies the 
type of place where the robot is currently located. Possible categories 
are: office, corridor, hall.

\item LM-detection (\textbf{LMD}): a memory based perceptual behavior that 
identifies specific LMs in the environment. Possible categories are a set 
of $m=80$ available visual LMs, as described in Section \ref{Sec:DL-Models}. 
\end{itemize}


\subsection{\label{Sec:Result1}Behavior training}

Input images consist of 160x120 pixels. We test using RGB and gray level 
images (BW), both schemes converge to suitable models, but BW achieves faster 
convergence. Therefore, we use BW images to train all behaviors, except LMD that 
uses RGB images. We normalize each input image by subtracting the mean and 
dividing by the standard deviation, both estimated over the training set. 
We use Adam as the optimization tool, keeping the recommended 
parameter values \cite{Adam:2014}. Initial learning rate is set to $10^{-4}$. 
Also, we apply batch-normalization \cite{BatchNormalization:2015} after every 
convolutional layer (except the last one).     

Table \ref{Table:Training} provides details about the datasets 
used to learn each behavior. To collect this data, we use virtual 
environments to render expert trajectories consisting of the robot executing 
each behavior. As an example, Figure \ref{Fig:CrossHall} shows a set of 
frames corresponding to a training instance used to fit the behavior 
\textit{cross-hall}. In this case, the robot crosses the hall continuing 
then its path using the right side corridor. As shown in Table 
\ref{Table:Training}, the size of each dataset is variable and mostly depends on 
the expected complexity of each behavior. Furthermore, during training, we use 
randomly sampled batches of 256 instances. 

\begin{figure}
\begin{center}
\includegraphics[width=8.7cm]{crossHall.png}
\end{center}
\caption{Sequential set of frames corresponding to samples of a 
training instance of behavior 
cross-hall. From left to right, the frames illustrate the robot entering, then 
crossing, and finally leaving the hall using the 
right side direction. } 
\label{Fig:CrossHall}
\end{figure}

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c}
\toprule
\multicolumn{5}{c}{\textbf{Navigational Behaviors}} \\
\bottomrule
  & Train: \#paths & Train: \#images & Test: \#trials & 
Accuracy\\
\bottomrule
\textbf{FC} & 150 & 46131 & 100 & 100\% \\
\textbf{IO} & 8000 & 221734 & 100 & 100\% \\
\textbf{OO} & 8000 & 259937 & 100 & 67\% \\
\textbf{OO-B} & 8000 & 259937 & 100 & 96\% \\
\textbf{CH} & 3000 & 248950 & 100 & 100\% \\
\textbf{CC} & 4000 & 123653 & 100 & 100\% \\

\toprule
\multicolumn{5}{c}{\textbf{Perceptual Behaviors}} \\
\bottomrule
  & - & Train: \#images & Test: \#images & 
Class. Acc.\\
\bottomrule
\textbf{PLD} & - &12945 & 1500 (Imgs) & 98.2\% \\
\textbf{LMD} & - & 38459 & 1500 (Imgs) & 96.7\% \\
\toprule
\end{tabular}
\end{center}
\caption{Details of the datasets used to train each behavior as well as the 
accuracy achieved on an independent test set. For navigational behaviors, we 
measure accuracy as the number of trials where the virtual robot successfully 
complete the goal of the behavior, ex. robot successfully leaves an office using 
the intended departing direction. For perceptual behaviors, we measure accuracy 
as the successful classification rate.}
\label{Table:Training}
\end{table}

In terms of perceptual behaviors, Table \ref{Table:Training} considers accuracy 
as the percentage of trials where the robot successfully completed 
the intended behavior, ex. crossing a corridor successfully using the intended 
departing direction. In terms of perceptual behaviors, accuracy 
is measured as the percentage of images where the model outputs a correct 
classification. For most behaviors, results in Table 
\ref{Table:Training} indicate a robust operation. The exception is 
behavior Out-Office (OO) that only succeed in 67\% of the trials. This poor 
performance is mainly due to the random scheme used to initialize the robot 
position, where in ocasions the robot starts in a position directly facing a 
close wall. In these cases, one will expect that the robot consistently rotates 
in one direction, searching for the position of the door to leave the 
office. However, the memoryless property of the CNN that is used to implement 
the behavior, can not handle this capability. As a result, robot usually 
starts wandering close to the wall entering a deadlock situation. While it 
is possible to use a recurrent model to implement this behavior, we decide to 
restrict the initial position of the robot so it always starts facing the 
initial direction of the path of the expert, which always points towards the 
door of the office. Introducing this simplification, we obtain behavior OO-B 
that is able to achieve a high robustness. 


\subsection{\label{Sec:Results2} Behavior Integration}
Next, we test the performance of the proposed approach to solve navigational 
tasks that require the integration of several behaviors. To conduct this 
experiment, we randomly generate 100 maps and for each map we randomly select 
10 independent tasks consisting on navigating between 2 different offices. This 
situation is similar to the case described in Figure \ref{twoApproaches}-b, 
where the robot needs to navigate from office $0_1$ to office $0_8$. For 
simplicity, we directly extract the graph representation from the known 
configuration of the environment. In a more general case, this map can be 
inferred by a guided presentation of the environment to the robot or by an 
initial unsupervised exploration phase. 

Tabla \ref{Table:Test} shows our results. Accuracy is measured as
the percentage of missions where the robot successfully reaches the intended 
goal location. As expected, the robot is 
able to successfully finish its mission in a significant proportion of the 
cases. Furthermore, the average length of 8.3 steps to complete each mission, 
which is equivalent to the timely combination of a similar number of behaviors, 
shows that the proposed approach is effective to control the selection and 
switching of behaviors. In terms of failure cases, a manual analysis reveals 
that these are mainly due to two problems. First, during robot navigation, the 
landmark detection behavior (LMD) occasionally fails to detect the landmark 
that identifies the entrance of the goal office. As a result, the robot misses 
to activate In-Office behavior (IO), traversing its last corridor 
until its end, to finally wonder without destination. This problem 
is related to the use of a first person camera view that is always pointing to 
the current heading direction of the robot. As a result, occasionally, this 
camera is not pointing in an expected direction missing the detection of a 
relevant landmark. A second failure case is due to the presence of repeated 
textural patterns in the virtual environment. In particular, the visual 
appearance of the view of a door just before leaving an office is highly similar 
to the view of the front door after leaving the office, as a result in some 
occasions the robot takes a wrong action, such as turning to face a 
hipothetical corridor before leaving the office. In practice, we 
believe that in a real implementation the previous two problems can be solved, 
and they do not constitute a major limitation to the viability of the proposed 
approach. 

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c}
\hline 
\#Maps & \#Missions/map & \#Missions & Av. Steps/mission & 
Acc.	\\
\hline\hline
100   & 10 & 1000 & 8.3 &  81.2\% \\ 
\hline
\end{tabular}
\end{center}
\caption{Performance of the proposed approach when robot needs to complete 
a mission consisting of navigating between 2 different offices. Accuracy is 
measured as the percentage of missions where the robot successfully reaches the 
intended goal location. We also report the average number of steps to complete 
a mission, which is equivalent to the average number of behaviors needed to 
complete the intended navigational plan.}
\label{Table:Test}
\end{table}



     
\section{\label{Sec:Discussion}APPENDIX: NOTATION}

\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline 
ooc& out of office &\\ 
\hline
& &\\ 
\hline
\end{tabular}
\end{center}
\label{Table:Notation}
\end{table}




 
